TrAISformer -- A Transformer Network with Sparse Augmented Data Representation and Cross Entropy Loss for AIS-based Vessel Trajectory Prediction

Vessel trajectory prediction plays a pivotal role in numerous maritime applications and services. While the Automatic Identification System (AIS) offers a rich source of information to address this task, forecasting vessel trajectory using AIS data remains challenging, even for modern machine learning techniques, because of the inherent heterogeneous and multimodal nature of motion data. In this paper, we propose a novel approach to tackle these challenges. We introduce a discrete, high-dimensional representation of AIS data and a new loss function designed to explicitly address heterogeneity and multimodality. The proposed model-referred to as TrAISformer-is a modified transformer network that extracts long-term temporal patterns in AIS vessel trajectories in the proposed enriched space to forecast the positions of vessels several hours ahead. We report experimental results on real, publicly available AIS data. TrAISformer significantly outperforms state-of-the-art methods, with an average prediction performance below 10 nautical miles up to ~10 hours.

==> bio2.tex <==
\begin{IEEEbiography}
    [{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/biography/Nguyen.jpg}}]{Duong Nguyen}
received the Dipl\^ome d'Ing\'enieur in machine learning from T\'el\'ecom Bretagne, the M.Sc. degree (summa cum laude) in signal and image processing from the University of Rennes 1, and the Ph.D. degree in machine learning from IMT Atlantique. His research interests focus on the study of machine learning (deep learning) for time series modeling and analysis, with applications to dynamical system identification and maritime traffic surveillance.

Duong Nguyen has published several papers on vessel trajectory analysis and anomaly detection. One of them has gained widespread adoption in industry and is being used as the foundation model to build maritime traffic anomaly detection systems. 
\end{IEEEbiography}

\begin{IEEEbiography}
    [{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/biography/Fablet.jpg}}]{Ronan Fablet} 
graduated with MSc. and Engineer degrees in Space Aeronautics and Applied Math from ISAE/SUPAERO in 1997 and with a PhD in Signal Processing and Computer Vision from University of Rennes/INRIA in 2001. After an INRIA postdoctoral fellowship with Brown University (RI, USA), he was a full-time research scientist at Ifremer (the French Institute for Sea Research) from 2003 to 2007. He joined IMT Atlantique in 2008 and currently holds a Professor position in the Mathematical and Electrical Engineering Department. He has been developing research activities at the interface between signal processing, machine learning and marine science. He has led national and international programs (e.g., EU STREP AFISA, ANR MN EMOCEAN, ANR ASTRID SESAME) and co-authored more than 200 articles and communications in peer-reviewed conferences and journals. His current research interest covers physics-informed deep learning, data-driven approaches to inverse problems, ocean remote sensing, and maritime surveillance.

\end{IEEEbiography}
